Latent Twins: A Framework for Scene Recognition and Fast Radiative Transfer Inversion in FORUM All-Sky Observations

The FORUM (Far-infrared Outgoing Radiation Understanding and Monitoring) mission will provide, for the first time, systematic far-infrared spectral measurements of Earth's outgoing radiation, enabling improved understanding of atmospheric processes and the radiation budget. Retrieving atmospheric states from these observations constitutes a high-dimensional, ill-posed inverse problem, particularly under cloudy-sky conditions where multiple-scattering effects are present. In this work, we develop a data-driven, physics-aware inversion framework for FORUM all-sky retrievals based on latent twins: coupled autoencoders for atmospheric states and spectra, combined with bidirectional latent-space mappings. A lightweight model-consistency correction ensures physically plausible cloud variable reconstructions. The resulting framework demonstrates potential for retrievals of atmospheric, cloud and surface variables, providing information that can serve as a prior, initial guess, or surrogate for computationally expensive full-physics inversion methods. It also enables robust scene classification and near-instantaneous inference, making it suitable for operational near-real-time applications. We demonstrate its performance on synthetic FORUM-like data and discuss implications for future data assimilation and climate studies.

==> disort.tex <==
In cloudy sky conditions, we must account for the scattering effects of cloud particles. This scattering can be characterized by the scattering cross-section, \(\sigma_{\text{scat}}\), which quantifies the probability that a photon is deflected (single scattering) and thereby reduces the intensity of the direct beam. This effect is considered alongside absorption, where the absorption cross-section is given by
\[
\sigma_{\text{abs}} = \frac{\alpha_\nu}{N},
\]
with \(N\) being the number density and \(\alpha_\nu\) the attenuation coefficient as defined in (\ref{eq:rt1}). However, a more sophisticated model (multiple scattering) also accounts for radiation arriving from other directions that is scattered into the beam.

Multiple scattering theory dates back to \cite{chandrasekhar1960}; here, we follow the approach of Stamnes \cite{stamnes1988} and his DIScrete Ordinate Radiative Transfer (DISORT) method, whose code \cite{stamnes2000} remains a standard reference. Under cloudy sky conditions, it is preferable to use the optical depth \(\od = \alpha_\nu z\) as the independent variable. For a light beam traveling in a direction defined by a polar angle \(\theta\) and an azimuth angle \(\varphi\), equation (\ref{eq:rt1}) can be recast as:
\begin{equation}\label{eq:rt2}
\begin{cases}
    \mu\,\dfrac{\mathrm{d} I_\nu}{\mathrm{d} \od}(\od,\mu,\varphi) = I_\nu(\od,\mu,\varphi) - S_\nu(\od,\mu,\varphi),\\[1ex]
    I_\nu((\od)_0)=(I_{\nu})_0,
\end{cases}
\end{equation}
where \(\mu = \cos(\theta)\), and the source function \(S_\nu\) now includes both the thermal emission from (\ref{eq:rt1}) and the additional scattering contributions. The source function is generally expressed as:
\begin{equation}\label{eq:source}
\begin{aligned}
S_\nu(\od,\mu,\phi)=&\frac{\omega_\nu(\od)}{4\pi}\int_0^{2\pi}\mathrm{d}\phi'\int_{-1}^{1}\mathrm{d}\mu'\,P_\nu(\od,\mu,\phi,\mu',\phi')\,I_\nu(\od,\mu',\phi')\\[1ex]
&+Q_\nu(\od,\mu,\phi),
\end{aligned}
\end{equation}
where the single scattering albedo,
\[
\omega_\nu(\od) = \frac{\sigma_{\text{scat}}}{\sigma_{\text{scat}}+\sigma_{\text{abs}}},
\]
describes the fraction of attenuation due to scattering, \(Q_\nu\) is the source term, and \(P_\nu\) is the phase function describing the angular scattering pattern of the cloud particles.

The source term \(Q_\nu(\od)\) is the sum of the thermal emission of the medium,
\[
Q_\nu^{(t)}(\od) = \bigl[1-\omega_\nu(\od)\bigr]B_\nu\bigl(T(\od)\bigr),
\]
and the contribution from an incoming beam, \(Q_\nu^{(b)}(\od,\mu,\phi)\). For a fixed beam direction \((\mu_0,\phi_0)\), the incoming beam can be related to the initial intensity \(I_0\) via the BLB law:
\begin{equation}\label{eq:incoming_beam}
Q_\nu^{(b)}(\od,\mu,\phi)=I_0\,\frac{\omega_\nu(\od)}{4\pi}\,P_\nu(\od,\mu,\phi,-\mu_0,\phi_0)\,\exp\Bigl(-\frac{\od}{\mu_0}\Bigr).
\end{equation}

The phase function is normalized such that
\begin{equation}\label{eq:phase_norm}
\frac{1}{4\pi}\int_0^{2\pi}\mathrm{d}\phi'\int_{-1}^{1}\mathrm{d}\mu'\,P_\nu(\od,\mu,\phi,\mu',\phi') = 1.
\end{equation}

If the phase function and the single scattering albedo are specified, equation (\ref{eq:rt1}) can in principle be solved for each fixed frequency \(\nu\). To obtain an explicit solution, equation (\ref{eq:rt1}) is expanded in a Fourier series with the following procedure, where the \(\nu\) suffix is dropped for simplicity.

The scattering is assumed to be isotropic, so that the phase function $P$ only depends on the plane angle $\Theta$ between the $(\mu,\phi)$ and $(\mu',\phi')$ directions. The phase function is then expanded in a series using Legendre polynomials
\begin{equation}\label{eq:leg}
P_l(x)=\frac{1}{2^ll!}\frac{d^l}{dx^l}\left[(x^2-1)^l\right].
\end{equation}
Also, from the spherical harmonics theory, the associated Legendre polynomials for a positive integer $m$ are defined as
\begin{equation}\label{eq:leg2}
P^m_l(x)=(-1)^m(1-x^2)^{m/2}\frac{d^m}{dx^m}P_l(x),\quad P^{-m}_l(x)=(-1)^m\frac{(l-m)!}{(l+m)!}P^m_l(x)
\end{equation}
Then the phase function can be written
\begin{equation}\label{eq:phase_leg}
P(\tau,\cos(\Theta))=\sum_{l=0}^{2N-1}(2l+1)g_l(\tau)P_l(\cos(\Theta)),
\end{equation}
where the $g_l(\tau)$ are given by
\begin{equation}\label{s1:eq:exp2}
g_l(\tau)=\frac{1}{2}\int_{0}^{\pi}P(\tau,\cos(\Theta))P_l(\cos(\Theta))\sin(\Theta)d\Theta.
\end{equation}
By setting
\begin{equation}\label{eq:phase3}
D^m(\tau,\mu,\mu')=\frac{\omega(\tau)}{2}\sum_{l=m}^{2N-1}(2l+1)g^m_l(\tau)P^m_l(\mu)P^m_l(\mu')
\end{equation}
the two-dimensional integral of equation (\ref{eq:source}) becomes
\begin{equation}\label{eq:phase4}
\sum_{m=0}^{2N-1}\left[\int_{-1}^{1}d\mu'I^m(\tau,\mu')D^m(\tau,\mu,\mu')\right]\cos[m(\phi_0-\phi)].
\end{equation}
The source term may also be decomposed in Fourier terms, by setting
\begin{equation}\label{eq:beam2}
\begin{aligned}
X_0^m(\tau,\mu)=&\frac{\omega(\tau)I_0}{4\pi}(2-\delta_{0m})\sum_{l=m}^{2N-1}(-1)^{l+m}(2l+1)g^m_l(\tau)P^m_l(\mu)P^m_l(\mu_0),\\ Q^m(\tau,\mu)=&X_0^m(\tau,\mu)\exp(-\tau/\mu)+\delta_{0m}Q^{(t)}(\tau).
\end{aligned}
\end{equation}
where $\delta_{ij}$ is the Kronecker delta. Then
\begin{equation}\label{s1:source2}
Q(\tau,\mu,\phi)=\sum_{m=0}^{2N-1}Q^m(\tau,\mu)\cos[m(\phi_0-\phi)],
\end{equation}
and we can finally replace the scattering problem (\ref{eq:rt1}-\ref{eq:phase_norm}) with a set of $2N$ independent integro-differential equations
\begin{equation}\label{eq:scat_int}
\mu \frac{dI^m(\tau,\mu)}{d\tau}=I^m(\tau,\mu,\phi)-\int_{-1}^1D^m(\tau,\mu,\mu')I^m(\tau,\mu')d\mu'-Q^m(\tau,\mu).
\end{equation}

From a numerical standpoint, the DISORT method \cite{stamnes2000} solves the scattering problem (\ref{eq:scat_int}) by using a Gaussian quadrature formula for the integral with nodes $\pm \mu_i$, $i=1,\ldots,N$
and weights $w_i$, obtaining
\begin{equation}\label{eq:scat_int2}
\mu_i \frac{dI^m(\tau,\mu_i)}{d\tau}=I^m(\tau,\mu_i,\phi)-\hspace{-1em}\sum_{\substack{j=-N,\ldots,N \\ j\neq 0}}\hspace{-1em}w_jD^m(\tau,\mu_i,\mu_j)I^m(\tau,\mu_j)-Q^m(\tau,\mu_i),\ i=\pm 1,\ldots,\pm n
\end{equation}
There is no analytical solution for (\ref{eq:scat_int}) because both the albedo and the phase function depend on $\tau$. The atmosphere is then discretized in a set of $L$ layers where the albedo and the phase function are constant, and the equations (\ref{eq:scat_int2}) are recast as a system of ordinary differential equations with the following definitions:
\begin{equation}\label{eq:mat_def}
\begin{aligned}
\bfI^\pm&=\{I^m(\tau,\pm \mu_i), i=1,\ldots,N\},\ \bfQ^\pm=\{Q^m(\tau,\pm \mu_i), i=1,\ldots,N\},\\
\bfM&=\{\mu_i\delta_{ij}, i,j=1,\ldots,N\},\ \bfQ'^\pm=\bfM^{-1}\bfQ^\pm\\
\bfW&=\{w_i\delta_{ij}, i,j=1,\ldots,N\},\\
\bfD^+&=\{D^m(\mu_i,\mu_j), i,j=1,\ldots,N\}=\{D^m(-\mu_i,-\mu_j), i,j=1,\ldots,N\},\\
\bfD^-&=\{D^m(-\mu_i,\mu_j), i,j=1,\ldots,N\}=\{D^m(\mu_i,-\mu_j), i,j=1,\ldots,N\},\\
\boldsymbol{\alpha}&=\bfM^{-1}\left(\bfD^+\bfW-\bfI\right),\ \boldsymbol{\beta}=\bfM^{-1}\bfD^-\bfW,
\end{aligned}
\end{equation}
so that (\ref{eq:scat_int2}) in each homogeneous layer becomes:
\begin{equation}\label{eq:system2}
\frac{d}{d\tau}\begin{bmatrix}\bfI^+\\ \bfI^-\end{bmatrix}=\begin{bmatrix}-\boldsymbol{\alpha}&-\boldsymbol{\beta}\\ \boldsymbol{\beta}&\boldsymbol{\alpha}\end{bmatrix}\begin{bmatrix}\bfI^+\\ \bfI^-\end{bmatrix}-
\begin{bmatrix}\bfQ'^+\\ \bfQ'^-\end{bmatrix}
\end{equation}
The system (\ref{eq:scat_int2}) is solved by first finding solutions of the homogeneous system in the form:
\begin{equation}\label{eq:eigen1}
\bfI^\pm=\bfG^\pm e^{-k\tau},{\textrm{where:}\  }\bfG^\pm=\begin{bmatrix}G(\pm\mu_1)\\\cdots\\G(\pm\mu_N)\end{bmatrix}.
\end{equation}
This leads to the following eigenvalue problem:
\begin{equation}\label{eq:eigen2}
\begin{bmatrix}\boldsymbol{\alpha}&\boldsymbol{\beta}\\ -\boldsymbol{\beta}&-\boldsymbol{\alpha}\end{bmatrix}\begin{bmatrix}\bfG^+\\ \bfG^-\end{bmatrix}=k\begin{bmatrix}\bfG^+\\ \bfG^-\end{bmatrix}
\end{equation}
for eigenvalues $k$ and eigenvectors $\bfG^\pm$. A particular solution of (\ref{eq:scat_int2}) can be found in the form
\begin{equation}\label{eq:part1}
I^m(\tau,\mu_i)=Z_0^m(\mu_i)e^{-\tau/\mu_0},
\end{equation}
where the $Z_0^m$ can be found by solving the following linear system:
\begin{equation}\label{eq:part2}
\sum_{\substack{j=-N,\ldots,N \\ j\neq 0}}\left[\left(1+\frac{\mu_j}{\mu_0}\right)\delta_{ij}-w_jD(\mu_i,\mu_j)\right]Z_0^m(\mu_j)=X_0^m(\mu_j).
\end{equation}
Finally, boundary conditions needs to be added, depending on the scanning geometry.

In practice, the effect of the scattering is to add an additional attenuation coefficient due to clouds which adds up with the effect of the atmospheric gases due to LBL law (\ref{eq:rt_sol}) that needs anyway to be calculated. In fact, one of the inputs of the DISORT method are the optical depths $-\alpha_\nu\Delta z$ of the atmospheric layers due to absorption. Once the total attenuation coefficients, \(\alpha_i\) for \(i=1,\ldots,L\), have been determined, the spectrum at the top of the atmosphere for a nadir-viewing instrument can be calculated using the standard radiative transfer equation \cite{zdunkowski2007}:
\begin{gather}\label{eq:RTE_discr}
\begin{split}
I(\tau_{L})=\Biggl[\, \epsilon \, B(T_{E}) + (1-\epsilon) \Bigl( \sum_{i=1}^{L} B(T_{i}) \, \Bigl(1 - \e^{-\alpha_{i}\Delta_i}\Bigr) \, \e^{-\sum_{j=1}^{i-1} \alpha_{j}\Delta_j} \Bigr) \Biggr] \e^{-\sum_{i=1}^{L} \alpha_{i}\Delta_i} \\
\quad +\sum_{i=1}^{L} B(T_{i}) \, \Bigl(1 - \e^{-\alpha_{i}\Delta_i}\Bigr) \, \e^{-\sum_{j=i+1}^{L} \alpha_{j}\Delta_j},
\end{split}
\end{gather}
where \(\epsilon\) is the emissivity, \(T_{E}\) is the surface temperature, \(T_i\) is the average temperature of layer \(i\), and \(\Delta_i\) is the geometrical thickness of layer \(i\).

The key issue of the DISORT method is the definition of the phase function $P(\tau,\cos(\Theta))$ that, as well as the single scattering albedo, depends on the type, the average dimension and the density of the particles that can be found in the cloud, the so-called particle habitat. The typical function used for this applications is the Mie function \cite{bohren1983}. The number $N$ of \emph{streams} depends on how well the phase function is approximated by the corresponding number of Legendre coefficients. The $\delta$-M transformation \cite{wiscombe1977} separates the phase function in a $\delta$ function for the forward direction and a residual phase function, that is hopefully reconstructed with less Legendre coefficients.

The DISORT is an accurate method, that is however very slow, even with its accelerated version \cite{sgheri2018}. An alternative way to parameterize the backscatter parameter, implemented in the code that will be used for calculating the training and test sets in this paper, is the Chou approximation \cite{chou1999}. Liquid and ice clouds are parametrized using particle content and size on each layer, and the effect is added as an additional attenuation coefficient.

